Coarse space preconditioning for Generalized Optimized Schwarz Methods. Part I: continuous case

The Generalized Optimized Schwarz Method (GOSM) originally proposed in [Claeys, 2021] is a variant of Depr\'es algorithm, a domain decomposition strategy for the solution of harmonic wave propagation problems. It imposes transmission conditions through interfaces by means of a non-local exchange operator. Conducting our analysis at the continuous level, in an infinite dimensional setting, we propose a coarse space construction for the preconditioning of the GOSM formulation, and provide estimates for the convergence of GMRes applied to the preconditioned equation.

==> macro.tex <==
\makeatletter
\newcommand\RedeclareMathOperator{%
  \@ifstar{\def\rmo@s{m}\rmo@redeclare}{\def\rmo@s{o}\rmo@redeclare}%
}
% this is taken from \renew@command
\newcommand\rmo@redeclare[2]{%
  \begingroup \escapechar\m@ne\xdef\@gtempa{{\string#1}}\endgroup
  \expandafter\@ifundefined\@gtempa
     {\@latex@error{\noexpand#1undefined}\@ehc}%
     \relax
  \expandafter\rmo@declmathop\rmo@s{#1}{#2}}
% This is just \@declmathop without \@ifdefinable
\newcommand\rmo@declmathop[3]{%
  \DeclareRobustCommand{#2}{\qopname\newmcodes@#1{#3}}%
}
\@onlypreamble\RedeclareMathOperator
\makeatother


\newcommand{\floor}[1]{\lfloor #1\rfloor}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\mrm}{\mathrm}
\newcommand{\mA}{\mathrm{A}}
\newcommand{\mK}{\mathrm{K}}
\newcommand{\mB}{\mathrm{B}}
\newcommand{\mL}{\mathrm{L}}
\newcommand{\mH}{\mathrm{H}}
\newcommand{\mJ}{\mathrm{J}}
\newcommand{\mU}{\mathrm{U}}
\newcommand{\mV}{\mathrm{V}}
\newcommand{\mW}{\mathrm{W}}
\newcommand{\mM}{\mathrm{M}}
\newcommand{\Id}{\mathrm{Id}}
\newcommand{\mD}{\mathrm{D}}
\newcommand{\mT}{\mathrm{T}}
\newcommand{\mS}{\mathrm{S}}
\newcommand{\mP}{\mathrm{P}}
\newcommand{\mR}{\mathrm{R}}
\newcommand{\mQ}{\mathrm{Q}}
\newcommand{\mX}{\mathrm{X}}
\newcommand{\mY}{\mathrm{Y}}
\newcommand{\mZ}{\mathrm{Z}}
\newcommand{\mbH}{\mathbb{H}}
\newcommand{\mbV}{\mathbb{V}}
\newcommand{\mbX}{\mathbb{X}}
\newcommand{\Vh}{\mathrm{V}_{h}}
\newcommand{\Wh}{\mathrm{W}_{h}}
\newcommand{\Qh}{\mathrm{Q}_{h}}
\newcommand{\VhO}{\mathrm{V}_{h,0}}
\newcommand{\mbVh}{\mathbb{V}_{h}}
\newcommand{\mbXh}{\mathbb{X}_{h}}
\newcommand{\infsup}{\mathop{\mrm{infsup}}}
\newcommand{\rref}{\textsc{r}}
\newcommand{\bell}{\boldsymbol{\ell}}

\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}

\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\bff}{\boldsymbol{f}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\bn}{\boldsymbol{n}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\bq}{\boldsymbol{q}}
\newcommand{\bl}{\boldsymbol{l}}
\newcommand{\bg}{\boldsymbol{g}}
\newcommand{\bd}{\boldsymbol{d}}
\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\bc}{\boldsymbol{c}}
\newcommand{\bb}{\boldsymbol{b}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bfff}{\mathbf{f}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfn}{\mathbf{n}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfq}{\mathbf{q}}
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\dir}{\textsc{d}}
\newcommand{\neu}{\textsc{n}}
\newcommand{\llangle}{\langle\!\langle}
\newcommand{\rrangle}{\rangle\!\rangle}
\newcommand{\lbr}{\lbrack}
\newcommand{\rbr}{\rbrack}

\newcommand{\ctru}{\mathfrak{u}}
\newcommand{\ctrv}{\mathfrak{v}}
\newcommand{\ctrw}{\mathfrak{w}}
\newcommand{\ctrp}{\mathfrak{p}}
\newcommand{\ctrq}{\mathfrak{q}}
\newcommand{\ctrf}{\mathfrak{f}}
\newcommand{\ctrg}{\mathfrak{g}}


%% \newcommand{\ctru}{\boldsymbol{u}}
%% \newcommand{\ctrv}{\boldsymbol{v}}
%% \newcommand{\ctrw}{\boldsymbol{w}}
%% \newcommand{\ctrp}{\boldsymbol{p}}
%% \newcommand{\ctrq}{\boldsymbol{q}}
%% \newcommand{\ctrf}{\boldsymbol{f}}
%% \newcommand{\ctrg}{\boldsymbol{g}}

\newcommand{\bfA}{\mathbf{A}}
\newcommand{\bfB}{\mathbf{B}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\bfP}{\mathbf{P}}
\newcommand{\bfQ}{\mathbf{Q}}
\renewcommand{\dim}{\mrm{dim}}
\newcommand{\Th}{\mathrm{T}_h}
\renewcommand{\div}{\mrm{div}}
\DeclareMathOperator{\T}{T} % Local Transmission operator

\DeclareMathOperator{\V}{\mathcal{V}_{\Gamma}} % weakly singular operator
\DeclareMathOperator{\K}{\mathcal{K}_{\Gamma}} % double layer potential or its adjoint
\DeclareMathOperator{\Kprime}{\tilde{\mathcal{K}}_{\Gamma}} % double layer potential adjoint
\DeclareMathOperator{\W}{\mathcal{W}_{\Gamma}} % hypersingular operator


%% \newcommand{\Bh}{\mathrm{B}_h}
%% \newcommand{\Ah}{\mathrm{A}_h}
%% \newcommand{\Sh}{\mathrm{S}_h}

\newcommand{\Bh}{\mathrm{B}}
\newcommand{\Ah}{\mathrm{A}}
\newcommand{\Sh}{\mathrm{S}}



\newcommand{\Ts}{\mT_{\textsc{s}}}
\newcommand{\Ps}{\mP_{\textsc{s}}}
\newcommand{\Range}{\mrm{Range}}


\newcommand{\calT}{\mathcal{T}}

\newcommand{\dof}{\mathrm{dof}}
\newcommand{\loc}{\mathrm{loc}}
\newcommand{\supp}{\mathrm{supp}}
\DeclareMathOperator{\diag}{diag} % diagonal



% Cite Left and Right Figures
\newcommand{\figpart}[2]{\cref{#1}~(#2)}

\DeclareMathOperator{\DtN}{DtN} % Dirichlet to Neumann operator


\newcommand{\Hdemi}{\mH^{1/2}(\Gamma)} % H^{1/2} space on Gamma (boundary)
\newcommand{\HMdemi}{\mH^{-1/2}(\Gamma)} % H^{-1/2} space on Gamma (boundary)

% \RedeclareMathOperator{\Re}{Re} % real part
% \RedeclareMathOperator{\Im}{Im} % imaginary part  Can not be used because \mrm{Im} already used to denote the image!
\renewcommand{\Re}{\mathfrak{Re}} % real part
\renewcommand{\Im}{\mathfrak{Im}} % imaginary part


%%%%%%%%%%%%%%%%%%%%%%%
\newtheorem{defn}{Definition}[section]
\newtheorem{lem}[defn]{Lemma}
\newtheorem{thm}[defn]{Theorem}
\newtheorem{prop}[defn]{Proposition}
\newtheorem{cor}[defn]{Corollary}
\newtheorem{rem}[defn]{Remark}
\newtheorem{example}[defn]{Example}
\newtheorem{asum}{Assumption}
\newtheorem{cond}[asum]{Condition}
\newtheorem{remark}{Remark}

